RED-Attack: Resource Efficient Decision based Attack for Machine Learning

Due to data dependency and model leakage properties, Deep Neural Networks (DNNs) exhibit several security vulnerabilities. Several security attacks exploited them but most of them require the output probability vector. These attacks can be mitigated by concealing the output probability vector. To address this limitation, decision-based attacks have been proposed which can estimate the model but they require several thousand queries to generate a single untargeted attack image. However, in real-time attacks, resources and attack time are very crucial parameters. Therefore, in resource-constrained systems, e.g., autonomous vehicles where an untargeted attack can have a catastrophic effect, these attacks may not work efficiently. To address this limitation, we propose a resource efficient decision-based methodology which generates the imperceptible attack, i.e., the RED-Attack, for a given black-box model. The proposed methodology follows two main steps to generate the imperceptible attack, i.e., classification boundary estimation and adversarial noise optimization. Firstly, we propose a half-interval search-based algorithm for estimating a sample on the classification boundary using a target image and a randomly selected image from another class. Secondly, we propose an optimization algorithm which first, introduces a small perturbation in some randomly selected pixels of the estimated sample. Then to ensure imperceptibility, it optimizes the distance between the perturbed and target samples. For illustration, we evaluate it for CFAR-10 and German Traffic Sign Recognition (GTSR) using state-of-the-art networks.

==> Sections/Sec2_Background.tex <==
\section{Background} \label{MAD}

In order to properly categorize the power of an adversary, every attack or defense has to assume some threat model \cite{DBLP:journals/corr/CarliniW16a}. A threat model is defined as a set of assumptions characterizing the freedom and strength of the adversary. Here we introduce the threat models currently assumed by the state-of-the-art attacks.

\textbf{White-Box Model}

Most attack algorithms proposed to date consider the white-box scenario in which the adversary has full knowledge of the architecture of the neural network, the trained weights and the gradients of the network. Under this assumption, the adversary can perform the back-propagation on the target network to compute the gradients of some loss metric. These gradients can then be used to find the optimal direction of perturbation to generate the adversarial example.
Examples of attacks which assume White-Box threat Models are:
\begin{enumerate}
    \item \textbf{FGSM Attack  \cite{goodfellow2014explaining} - }FGSM (Fast Gradient Sign Method) first defines a loss function, \(L\) and then computes the sign of the gradient of \(L\) with respect to each pixel \(x\) in the input image \(X\). If the classifier is characterized by \(f\),
    \[L = (f(X) - f(target))^2\]
    \[\Delta_x = \epsilon \times sign(\frac{\partial L}{\partial x_X})\]
    \[X_{adv} = X + \Delta_x\]
    \item \textbf{I-FGSM Attack \cite{DBLP:journals/corr/KurakinGB16} - }I-FGSM (Iterative FGSM) is an iterative variant of FGSM attack which computes the sign of the gradients of the loss function at current adversarial instance for each iteration and updates the adversarial instance accordingly. Mathematically,
    \[L = (f(X_{adv}) - f(target))^2\]
    \[\Delta_{adv} = \frac{\epsilon}{n} \times \frac{\partial L}{\partial x_{adv}}\]
    \[X_{adv} = X_{adv} + \Delta_{adv}\]
    \item \textbf{JSMA \cite{DBLP:journals/corr/PapernotMJFCS15} - }JSMA (Jacobian Saliency Map Attack) computes the gradient matrix of the loss with respect to the input image and introduces perturbation in the pixel bearing maximum value in the gradient matrix. This is repeated until the maximum number of pixels (predefined by the threshold have been perturbed) or a successful adversarial example is generated.
    \item \textbf{CW Attack - }CW (Carlini-Wagner) Attack defines several useful cost functions which can be minimized using different hyper-parameters to get different adversarial examples. The flexible definition of CW attack makes it one of the strongest and most useful attack in the white-box scenario. One of the most commonly used cost function is given below:
    \[cost = c \times (f(X_{adv}) - f(target))^2 + \sum{(X - X_{adv})^2}\]
\end{enumerate}

There are several other white-box attacks e.g. One-Pixel Attack, Universal Adversarial Perturbation, DeepFool, PGD-Attack. However, white-Box Attacks are often impractical in real scenarios because of their assumption that the adversary has complete knowledge of the network architecture and its parameters' values.

\textbf{Black-Box Model}

A harder but more practical models are built by limiting the capability of the adversary regarding the knowledge of the target network. Black-box models assume that the adversary has no knowledge of the target architecture. However, the adversary may query the target network for a given image. Based on the knowledge of the adversary the black-box scenario can be further divided into three categories.
\begin{enumerate}
    \item \textbf{Prediction Vector is exposed -} In this scenario the adversary has access to the conditional probability of each class as computed by the target network, given an input image. We call this ``Simple Black-Box (SBB)'' settings.
    \item \textbf{Probability of the k-classes is exposed -} This model further limits the capability of the adversary and allows it to have access to the conditional probability of only top k-classes, given an input image. We call this model ``Limited Black-Box (LBB)'' settings. Zeroth-Order Optimization based Attack \cite{DBLP:conf/ccs/ChenZSYH17}, Gen-Attack \cite{DBLP:journals/corr/abs-1805-11090}, Gradient-Estimation Attack assume this threat model.
    \item \textbf{Only the decision label is exposed -} In terms of knowledge, this threat model implies the most strict conditions on the adversary by assuming that the target network only exposes its top-k decisions without exposing their probabilities. Threat models based on such assumptions may be called ``Very Limited Black-Box (VLBB)'' settings. Decision-based attack \cite{DBLP:journals/corr/abs-1712-04248} is one such example which utilize random walk along the boundary to arrive at an adversarial example. However, decision-based attacks are quite in-efficient in terms of the number of queries and come with no guarantee of convergence.
\end{enumerate}
We may put further constraints on the adversary by limiting the number of queries, an adversary is allowed to make. Such settings may be regarded as ``Query-Limited Settings''.

In this paper, we assume the ``Very Limited Black-Box (VLBB)'' threat model, as it presents a scenario applicable to many real-world secure Machine Learning System settings. To further limit our knowledge, we assume k = 1 for our experiments i.e. our target network only exposes the label of the class with the highest probability. We evaluate our results for the ``query-limited settings'' where maximum number of queries an adversary is allowed to make is pre-defined.

==> Sections/Sec3_Motivational_Analysis_Discussion.tex <==
\section{Motivational Analysis and Discussion} \label{MAD}

Computing an adversarial example under Very Limited Black-Box threat model is a very challenging problem because such threat models do not reveal the stochastic gradients of the target network. Almost all of the state-of-the-art black box attacks, estimate the stochastic gradient of the network, by randomly perturbing the input pixels and studying the change in the output probability vector. All such attacks are rendered ineffective under VLBB settings.
To further verify our hypothesis, we conduct an initial experiment to study the effects of Black-Output on Zeroth-Order Optimization based Attack \cite{DBLP:conf/ccs/ChenZSYH17}. We reuse the open source code provided by \cite{DBLP:conf/ccs/ChenZSYH17}. We modify the implementation of the black-box model in \cite{DBLP:conf/ccs/ChenZSYH17} by performing one-hot encoding on the output of the Classifier. The results of ZOO Attack are shown in Table 1.


Generating an adversarial example under Label-Only settings requires an adversary to use iterative discrete optimization to arrive at a suitable adversarial example. Considering the complexity of the problem, in our knowledge, decision-based attack is the only attack that has been proposed, to date. Decision-based attack is a powerful adversarial attack which generates adversarial examples without having to require the probabilities of the output (See Fig \ref{fig:DF})

However decision-based attack is not feasible in resource limited scenarios, because it generates batches of images at different iterations to work successfully. Further, it initializes an input example by adding a uniform noise of increasing standard deviation in the clean image to generate an initial adversarial example. One major disadvantage of this approach is that it does not guarantee arrival at an initial adversarial point.

We seek to overcome both of these limitations of the Decision-based attacks by modifying it to successfully work on strictly resource critical scenarios and providing it with an initial direction which guarantees an initial adversarial example to be found, at the cost of the number of queries. In addition to that, we propose an efficient update process that significantly increases the quality of adversarial examples. For practical purposes, we attack a model trained on a well-known German Traffic Sign Recognition Benchmark (GTSRB) data set and prove the unreliability of Machine Learning Algorithms under practical settings.

==> Sections/Z_Sec3_QuSecNets.tex <==
\section{Quantization-based Defense for DNN} \label{QusecNets}
In this section, we discuss the proposed methodology, QuSecNets, which exploits the quantization to develop a defense mechanism against the adversarial attack in CNNs. The proposed methodology consists of the following steps, as shown in Fig.~\ref{fig:QuSecNets}.

\begin{enumerate}[leftmargin=*]
    \item First, we select a DNN model and the quantization methods based on the targeted vulnerabilities, input dataset and applications.
    
    \item Afterwards, we design and integrate the quantization layer within the selected DNN model. This quantization layer has one-to-one relation with the input layer, i.e., for each input pixel there is a seperate quantization function. This function is defined as the average value of $``n''$ sigmoid functions $``S(x,\ t_k)''$ (See Fig.~\ref{fig:QuSecNets}) and can be formulated as:
    \begin{equation}
      y = S(x,t_k) = \frac{1}{n-1} \times \sum_{k=1}^{n} \Bigg(\frac{1}{1+e^{-z(x-t_k)}}\Bigg)
    \label{Eq:eq1}
    \end{equation}
    Where $x$, $z$ and $t_k$ are the intensity of a single pixel from input image, the scalar constant and the threshold values which \textit{may} (in variable quantization) or \textit{may not} (in constant quantization) be trained, respectively. Moreover, n represents the number of quantization levels, e.g., if the number of quantization levels is 2, all the values below 0.5 are pushed towards 0, while those above or equal to 0.5 are pushed towards the maximum value, which is 1 in our case.
    
    \item After integrating the quantization layer in the CNN, we train the modified network, depending upon the quantization methodology. For example, in case of constant quantization, we do not train the quantization layer. However, in case of variable quantization we propose to utilize the backpropagation methodology.
    
\end{enumerate}

\begin{figure}[t!]
	\centering
	\includegraphics[width=1\linewidth]{Figs/QuSecNets.pdf} 
	\caption{\textit{Proposed Methodology, QuSecNets, to design quantization-aware secure CNNs}}
	\label{fig:QuSecNets}
\end{figure} 

\subsection{Training the Quantization Layer}
In case of variable quantization, we need to train the thresholds $(t_k)$ based on the output prediction/classification probabilities of the DNNs. Therefore, first we define a cost function to identify the difference between the actual and targeted predictions. 
    \begin{equation}
      cost = \frac{1}{c} \times \sum_{c=1}^{C} ( - P(x=c_{acc}))^2
    \label{Eq:eq2}
    \end{equation}
Where, $P(x=c_{acc})$ and $P(x=c)$represent the probability of input x to be classified as any class $c_{acc}$ and actual class ``c'', respectively. Similar to the back-propagation algorithm in CNN training, the threshold of the quantization layer can be trained by minimizing the cost function (Equation (~\ref{Eq:eq3})):
    \begin{equation}
        t_{k,new} =  t_{k,old} - \eta \frac{\partial (cost)}{\partial (t_{k,old})}
        \label{Eq:eq3}
    \end{equation}
Where, by chain rule,    
    \begin{equation}
         \frac{\partial (cost)}{\partial (t_{k,old})} = \frac{\partial (cost)}{\partial y} \times \frac{\partial y}{\partial (t_{k,old})}
        \label{Eq:eq4}
    \end{equation}
    
    \begin{equation}
         \frac{\partial y}{\partial (t_{k,old})} =  \Bigg( \sum_{k} \frac{-1}{n-1} \times z \times y_k \times (1-y_k)\Bigg)
        \label{Eq:eq5}
    \end{equation}
    
    \begin{equation}
        \frac{\partial (cost)}{\partial y_k} = \sum_{n} (w_{nk} \times \delta_n) = \Delta_k
        \label{Eq:eq6}
    \end{equation}
Where, $y_k$ is the output of the sigmoid function and $``\delta_k''$ denotes the sensitivity of $y_k$ for all the variables in the first convolutional layer of the DNN defined by the backpropagation. Thus, the change in cost function is determined by the following equation.
    \begin{equation}
        \frac{\partial (cost)}{\partial (t_{k,old})} = \Bigg(\sum_{k} \Delta_k\Bigg) \times \Bigg(\sum_{k} \frac{-1}{n-1} \times z \times y_k \times (1-y_k)\Bigg)
        \label{Eq:eq7}
    \end{equation}
By combining the Equations~\ref{Eq:eq3} and~\ref{Eq:eq7}, the training equation for quantization threshold is modeled as:   
    \begin{equation}
        t_{k,new} =  t_{k,old} - \eta \times \Bigg(\sum_{k} \Delta_k\Bigg) \times \Bigg(\sum_{k} \frac{-1}{n-1} \times z \times y_k \times (1-y_k)\Bigg)
        \label{Eq:eq8}
    \end{equation}
